On Divergence Measures for Training GFlowNets

Generative Flow Networks (GFlowNets) are amortized inference models designed to sample from unnormalized distributions over composable objects, with applications in generative modeling for tasks in fields such as causal discovery, NLP, and drug discovery. Traditionally, the training procedure for GFlowNets seeks to minimize the expected log-squared difference between a proposal (forward policy) and a target (backward policy) distribution, which enforces certain flow-matching conditions. While this training procedure is closely related to variational inference (VI), directly attempting standard Kullback-Leibler (KL) divergence minimization can lead to proven biased and potentially high-variance estimators. Therefore, we first review four divergence measures, namely, Renyi-$\alpha$'s, Tsallis-$\alpha$'s, reverse and forward KL's, and design statistically efficient estimators for their stochastic gradients in the context of training GFlowNets. Then, we verify that properly minimizing these divergences yields a provably correct and empirically effective training scheme, often leading to significantly faster convergence than previously proposed optimization. To achieve this, we design control variates based on the REINFORCE leave-one-out and score-matching estimators to reduce the variance of the learning objectives' gradients. Our work contributes by narrowing the gap between GFlowNets training and generalized variational approximations, paving the way for algorithmic ideas informed by the divergence minimization viewpoint.

==> tables/ablation.tex <==
\begin{table}[hbtp!]
\caption{Expected calibration error (mean and standard deviation). The best ECE results found for each GNN are highlighted in \textcolor{blue}{blue}. In most cases, \texttt{IN-N-OUT} outperforms the baseline by a considerable margin.}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l l r r r}
\toprule
\color{black} & \textbf{Model} \color{black} & \textbf{Uncalibrated} \color{black} & \textbf{Emb.+MLP} \color{black} & \textbf{{IN-N-OUT}} \\ 
\midrule
 \parbox[t]{5mm}{\multirow{3}{*}{\rotatebox[origin=c]{0}{Cite}}}
 \color{black} & VGAE \color{black} & 14.00 \color{gray} $\pm$ 0.67 \color{black} & 4.92 \color{gray} $\pm$ 1.06 \color{black} & \textbf{\color{blue}4.19} \color{gray} $\pm$ 0.65 \\
 \color{black} & SAGE \color{black} & 14.52 \color{gray} $\pm$ 1.89 \color{black} & \textbf{\color{blue}2.62} \color{gray} $\pm$ 0.62 \color{black} & 3.79 \color{gray} $\pm$ 1.98 \\
 \color{black} & PEG \color{black} & 28.39 \color{gray} $\pm$ 1.59 \color{black} & 17.75 \color{gray} $\pm$ 1.21 \color{black} & \textbf{\color{blue}12.02} \color{gray} $\pm$ 0.98 \\
\midrule
 \parbox[t]{5mm}{\multirow{3}{*}{\rotatebox[origin=c]{0}{Pub}}}
 \color{black} & VGAE \color{black} & 20.41 \color{gray} $\pm$ 0.64 \color{black} & 3.01 \color{gray} $\pm$ 1.16 \color{black} & \textbf{\color{blue}1.85} \color{gray} $\pm$ 0.37  \\
 \color{black} & SAGE \color{black} & 18.78 \color{gray} $\pm$ 1.42 \color{black} & 4.16 \color{gray} $\pm$ 1.47 \color{black} &  \textbf{\color{blue}3.01} \color{gray} $\pm$ 1.32 \\
\color{black} & PEG \color{black} & 20.49 \color{gray} $\pm$ 1.31 \color{black} & 8.90 \color{gray} $\pm$ 0.89 \color{black} & \textbf{\color{blue}8.21} \color{gray} $\pm$ 0.75 \\
\midrule
 \parbox[t]{5mm}{\multirow{3}{*}{\rotatebox[origin=c]{0}{TW}}}
 \color{black} & VGAE \color{black} & 16.32 \color{gray} $\pm$ 0.20 \color{black} & 4.81 \color{gray} $\pm$ 1.56 \color{black} & \textbf{\color{blue}1.50} \color{gray} $\pm$ 0.44 \\
 \color{black} & SAGE \color{black} & 16.84 \color{gray} $\pm$ 2.84 \color{black} & 4.06 \color{gray} $\pm$ 1.75 \color{black} & \textbf{\color{blue}1.53} \color{gray} $\pm$ 0.89 \\
 \color{black} & PEG \color{black} & 7.90 \color{gray} $\pm$ 0.91 \color{black} & 2.95 \color{gray} $\pm$ 0.59 \color{black} & \textbf{\color{blue}2.21} \color{gray} $\pm$ 0.51 \\
\midrule
 \parbox[t]{7mm}{\multirow{3}{*}{\rotatebox[origin=c]{0}{Chame}}}
 \color{black} & VGAE \color{black} & 7.52 \color{gray} $\pm$ 1.63 \color{black} & 3.57 \color{gray} $\pm$ 1.19 \color{black} & \textbf{\color{blue}1.07} \color{gray} $\pm$ 0.34 \\
 \color{black} & SAGE \color{black} & 5.98 \color{gray} $\pm$ 3.61 \color{black} & 3.99 \color{gray} $\pm$ 1.45 \color{black} & \textbf{\color{blue}2.46} \color{gray} $\pm$ 0.86 \\
 \color{black} & PEG \color{black} & 4.44 \color{gray} $\pm$ 0.24 \color{black} & 2.14 \color{gray} $\pm$ 0.21 \color{black} & \textbf{\color{blue}1.66} \color{gray} $\pm$ 0.36 \\
\midrule
  \parbox[t]{7mm}{\multirow{3}{*}{\rotatebox[origin=c]{0}{Alpha}}}
  \color{black} & VGAE \color{black} & 20.36 \color{gray} $\pm$ 1.53 \color{black} &  \textbf{\color{blue}7.12} $\pm$ \color{gray} 1.19  \color{black} & 8.42 $\pm$ \color{gray} 0.68\\
  \color{black} & SAGE \color{black} & 21.26 $\pm$ \color{gray} 1.37 \color{black} & 7.82 $\pm$ \color{gray}  1.45 \color{black} & \textbf{\color{blue}6.68} $\pm$ \color{gray} 0.91\\
  \color{black} & PEG \color{black} & 13.91 $\pm$ \color{gray} 1.13 \color{black} & \textbf{\color{blue}7.62} $\pm$ \color{gray} 1.76 \color{black} & 9.78 $\pm$ \color{gray} 0.89\\
\bottomrule
\end{tabular}
}
\label{tab:ablation}
% \vspace{-0.35cm}
\end{table}

==> tables/details_datasets.tex <==
\begin{table}[H]
\centering
\caption{Summary statistics of the datasets.}
\adjustbox{width=\linewidth}{
\begin{tabular}{lcccc}
\toprule
\textbf{Dataset} & \textbf{\# Nodes} & \textbf{\# Edges} & \textbf{\# Feat.} & \textbf{\# Labels}\\
\midrule
Cora & 2708 & 10556 & 1433 & 7 \\
PubMed & 19717 & 88648 & 500 & 3\\
Citeseer & 3327 & 9104 & 3703 & 6\\
%Twitch-RU & 4385 & 67148 & 128 & 2\\
Twitch & 1912 & 57905 & 128 & 2\\
Chameleon & 2277 & 39730 & 2325 & 5\\
Bitcoin-Alpha & 3783 & 28248 & 8 & 2\\
Bitcoin-OTC & 5881 & 42984 & 8 & 2\\
OGBL-DDI & 4267 & 1334889 & 5 & 2\\ 	
OGBL-Collab & 235868 & 1285465 & 128 & 2\\ 		
\bottomrule
\end{tabular}
}
\label{tab:details_datasets}
\end{table}

==> tables/ece_results.tex <==
\begin{table*}[ht!]
\centering
\caption{Expected calibration error (mean and std deviation). The best ECE results found for each GNN are highlighted in \textcolor{blue}{blue} (the lower the value, the better the model). Notably, \texttt{IN-N-OUT} outperforms the baselines in $\approx83\%$ of the cases.}  

% \adjustbox{width=\textwidth}{
\begin{tabular}{llrrrrrrrr}
\toprule
\color{black} & \textbf{Model} \color{black} & \textbf{ Uncalibrated} \color{black} & \textbf{Iso} \color{black} & \textbf{ Temp} \color{black} & \textbf{ BBQ} \color{black} & \textbf{ Hist} \color{black} & \textbf{ IN-N-OUT}\\ 
\toprule

 \parbox[t]{5mm}{\multirow{6}{*}{\rotatebox[origin=c]{0}{Cora}}}
 \color{black} & VGAE \color{black} & 15.02 \color{gray} $\pm$ 0.76 \color{black} & 6.88 \color{gray} $\pm$ 1.72 \color{black} & 12.62 \color{gray} $\pm$ 1.79 \color{black} & 7.09 \color{gray} $\pm$ 1.09 \color{black} & 6.14 \color{gray} $\pm$ 0.76 \color{black} & \textbf{ \color{blue}3.33} \color{gray} $\pm$ 0.67\\
 
 \color{black} & SAGE \color{black} & 17.23 \color{gray} $\pm$ 1.74 \color{black} & 17.36 \color{gray} $\pm$ 1.84 \color{black} & 17.20 \color{gray} $\pm$ 1.47 \color{black} & 17.66 \color{gray} $\pm$ 1.10 \color{black} & 17.61 \color{gray} $\pm$ 1.19 \color{black} & \textbf{ \color{blue}6.84} \color{gray} $\pm$ 0.48\\
 
 \color{black} & PEG \color{black} & 27.91 \color{gray} $\pm$ 0.60 \color{black} & 27.65 \color{gray} $\pm$ 1.34 \color{black} & 23.90 \color{gray} $\pm$ 1.55 \color{black} & 27.30 \color{gray} $\pm$ 1.40 \color{black} & 27.43 \color{gray} $\pm$ 1.89  \color{black} & \textbf{ \color{blue}11.53} \color{gray} $\pm$ 1.40\\
 
 \color{black} & GIN \color{black} & 15.07 \color{gray} $\pm$ 1.29 \color{black} & 16.66 \color{gray} $\pm$ 1.62 \color{black} & 14.23 \color{gray} $\pm$ 1.63 \color{black} & 16.36 \color{gray} $\pm$ 1.90 \color{black} & 16.63 \color{gray} $\pm$ 1.87 \color{black} & \textbf{ \color{blue}4.05} \color{gray} $\pm$ 1.31\\

 \color{black} & GCN \color{black} & 18.34 \color{gray} $\pm$ 1.13 \color{black} & 12.62 \color{gray} $\pm$ 0.97 \color{black} & 15.96 \color{gray} $\pm$ 1.11 \color{black} & 12.13 \color{gray} $\pm$ 1.30 \color{black} & 12.62 \color{gray} $\pm$ 1.08 \color{black} & \textbf{ \color{blue}6.90} \color{gray} $\pm$ 0.79\\

 \color{black} & SEAL \color{black} & 4.89 \color{gray} $\pm$ 0.18 \color{black} & 3.27 \color{gray} $\pm$ 0.15 \color{black} & 3.99 \color{gray} $\pm$ 0.66 \color{black} & 3.63 \color{gray} $\pm$ 0.24 \color{black} & 3.58 \color{gray} $\pm$ 0.20 \color{black} & \textbf{ \color{blue}2.41} \color{gray} $\pm$ 0.36\\
 
\midrule

 \parbox[t]{5mm}{\multirow{6}{*}{\rotatebox[origin=c]{0}{Cite}}}
 \color{black} & VGAE \color{black} & 14.00 \color{gray} $\pm$ 0.67 \color{black} & 5.52 \color{gray} $\pm$ 1.81 \color{black} & 18.57 \color{gray} $\pm$ 1.86 \color{black} & 5.14 \color{gray} $\pm$ 1.29 \color{black} & 5.02 \color{gray} $\pm$ 1.36 \color{black} & \textbf{ \color{blue}4.19} \color{gray} $\pm$ 0.65\\
 
 \color{black} & SAGE \color{black} & 14.52 \color{gray} $\pm$ 1.89 \color{black} & 18.81 \color{gray} $\pm$ 1.14 \color{black} & 12.86 \color{gray} $\pm$ 1.56 \color{black} & 18.64 \color{gray} $\pm$ 1.90 \color{black} & 17.88 \color{gray} $\pm$ 1.82 \color{black} & \textbf{ \color{blue}3.79} \color{gray} $\pm$ 1.98\\
 
 \color{black} & PEG \color{black} & 28.39 \color{gray} $\pm$ 1.59 \color{black} & 25.15 \color{gray} $\pm$ 1.74 \color{black} & 22.30 \color{gray} $\pm$ 1.35 \color{black} & 24.82 \color{gray} $\pm$ 1.76 \color{black} & 24.93 \color{gray} $\pm$ 0.56 \color{black} & \textbf{ \color{blue}12.02} \color{gray} $\pm$ 0.98\\
 
 \color{black} & GIN \color{black} & 15.69 \color{gray} $\pm$ 1.89 \color{black} & 23.86 \color{gray} $\pm$ 2.96 \color{black} & 13.98 \color{gray} $\pm$ 1.96 \color{black} & 23.80 \color{gray} $\pm$ 2.65 \color{black} & 23.30 \color{gray} $\pm$ 2.09 \color{black} & \textbf{ \color{blue}2.20} \color{gray} $\pm$ 0.86\\

 \color{black} & GCN \color{black} & 16.84 \color{gray} $\pm$ 1.62 \color{black} & 12.55 \color{gray} $\pm$ 1.43 \color{black} & 14.37 \color{gray} $\pm$ 1.19 \color{black} & 11.98 \color{gray} $\pm$ 1.59 \color{black} & 10.80 \color{gray} $\pm$ 1.62 \color{black} & \textbf{ \color{blue}6.06} \color{gray} $\pm$ 1.23\\

   \color{black} & SEAL \color{black} & 4.22 \color{gray} $\pm$ 0.31 \color{black} & 3.59 \color{gray} $\pm$ 0.49 \color{black} & 3.67 \color{gray} $\pm$ 0.35 \color{black} & 3.62 \color{gray} $\pm$ 0.30 \color{black} & 3.50 \color{gray} $\pm$ 0.24 \color{black} & \textbf{ \color{blue}2.93} \color{gray} $\pm$ 0.28\\
   
\midrule

 \parbox[t]{5mm}{\multirow{6}{*}{\rotatebox[origin=c]{0}{Pub}}}
 \color{black} & VGAE \color{black} & 20.41 \color{gray} $\pm$ 0.64 \color{black} & 3.04 \color{gray} $\pm$ 1.52 \color{black} & 20.83 \color{gray} $\pm$ 1.86 \color{black} & 2.22 \color{gray} $\pm$ 1.59 \color{black} &  \color{black}2.20 \color{gray} $\pm$ 1.97 & \textbf{\color{blue}1.85} \color{gray} $\pm$ 0.37\\
 
 \color{black} & SAGE \color{black} & 18.78 \color{gray} $\pm$ 1.42 \color{black} & 4.93 \color{gray} $\pm$ 1.41 \color{black} & 13.95 \color{gray} $\pm$ 1.72 \color{black} & 4.95 \color{gray} $\pm$ 1.57 \color{black} & 4.83 \color{gray} $\pm$ 1.32 \color{black} & \textbf{ \color{blue}3.01} \color{gray} $\pm$ 1.32\\
 
\color{black} & PEG \color{black} & 20.49 \color{gray} $\pm$ 1.31 \color{black} & 20.31 \color{gray} $\pm$ 1.93 \color{black} & 20.34 \color{gray} $\pm$ 1.28 \color{black} & 20.22 \color{gray} $\pm$ 0.28 \color{black} & 20.00 \color{gray} $\pm$ 1.39 \color{black} & \textbf{ \color{blue}8.21} \color{gray} $\pm$ 0.75\\

 \color{black} & GIN \color{black} & 15.33 \color{gray} $\pm$ 1.34 \color{black} & 12.72 \color{gray} $\pm$ 1.30 \color{black} & 14.96 \color{gray} $\pm$ 1.08 \color{black} & 12.66 \color{gray} $\pm$ 1.34 \color{black} & 12.67 \color{gray} $\pm$ 1.12 \color{black} & \textbf{ \color{blue}3.73} \color{gray} $\pm$ 0.89\\

 \color{black} & GCN \color{black} & 20.98 \color{gray} $\pm$ 1.79 \color{black} & 3.54 \color{gray} $\pm$ 1.97 \color{black} & 9.13 \color{gray} $\pm$ 1.97 \color{black} & \textbf{ \color{blue}3.34} \color{gray} $\pm$ 1.68 \color{black} & 3.44 \color{gray} $\pm$ 1.75 \color{black} & 4.44 \color{gray} $\pm$ 1.46\\

 \color{black} & SEAL \color{black} & 4.32 \color{gray} $\pm$ 0.33 \color{black} & 4.10 \color{gray} $\pm$ 0.17 \color{black} & 4.04 \color{gray} $\pm$ 0.16 \color{black} & 3.82 \color{gray} $\pm$ 0.48 \color{black} & 4.13 \color{gray} $\pm$ 0.32 \color{black} & \textbf{ \color{blue}2.42} \color{gray} $\pm$ 0.34\\
   
\midrule

 \parbox[t]{5mm}{\multirow{5}{*}{\rotatebox[origin=c]{0}{Twitch}}}
 \color{black} & VGAE \color{black} & 16.32 \color{gray} $\pm$ 0.20 \color{black} & 1.84 \color{gray} $\pm$ 1.10 \color{black} & 16.17 \color{gray} $\pm$ 1.45 \color{black} & 1.72 \color{gray} $\pm$ 1.13 \color{black} & 1.66 \color{gray} $\pm$ 1.24 \color{black} & \textbf{ \color{blue}1.50} \color{gray} $\pm$ 0.44\\
 
 \color{black} & SAGE \color{black} & 16.84 \color{gray} $\pm$ 2.84 \color{black} & 2.17 \color{gray} $\pm$ 1.37 \color{black} & 23.96 \color{gray} $\pm$ 1.53 \color{black} & 2.08 \color{gray} $\pm$ 1.14 \color{black} & 1.90 \color{gray} $\pm$ 1.42 \color{black} & \textbf{ \color{blue}1.53} \color{gray} $\pm$ 0.89\\
 
 \color{black} & PEG \color{black} & 7.90 \color{gray} $\pm$ 0.91 \color{black} & 5.36 \color{gray} $\pm$ 1.19 \color{black} & 5.81 \color{gray} $\pm$ 1.19 \color{black} & 5.35 \color{gray} $\pm$ 1.11 \color{black} & 5.38 \color{gray} $\pm$ 0.09 \color{black} & \textbf{ \color{blue}2.21} \color{gray} $\pm$ 0.51\\
 % \color{black} & SEAL \color{black} &  \color{gray} $\pm$  \color{black} &  \color{gray} $\pm$  \color{black} &  \color{gray} $\pm$  \color{black} &  \color{gray} $\pm$  \color{black} &  \color{gray} $\pm$  \color{black} & \textbf{ \color{blue} \color{blue} \color{gray} $\pm$ }\\

 \color{black} & GIN \color{black} & 17.86 \color{gray} $\pm$ 2.13 \color{black} & 1.91 \color{gray} $\pm$ 0.97 \color{black} & 13.78 \color{gray} $\pm$ 2.36 \color{black} & \textbf{\color{blue}1.85} \color{gray} $\pm$ 0.96 \color{black} & 1.86 \color{gray} $\pm$ 0.78 \color{black} & 2.69 \color{gray} $\pm$ 0.96\\

 \color{black} & GCN \color{black} & 16.09 \color{gray} $\pm$ 1.59 \color{black} & 2.56 \color{gray} $\pm$ 0.96 \color{black} & 6.79 \color{gray} $\pm$ 1.12 \color{black} & 1.66 \color{gray} $\pm$ 0.93 \color{black} & \textbf{\color{blue}1.61} \color{gray} $\pm$ 0.97 \color{black} & 4.16 \color{gray} $\pm$ 1.13\\
 
% \midrule

%  \parbox[t]{5mm}{\multirow{5}{*}{\rotatebox[origin=c]{0}{RU}}}
%  \color{black} & VGAE \color{black} & 16.92 \color{gray} $\pm$ 0.75 \color{black} & 2.15 \color{gray} $\pm$ 1.30 \color{black} & 12.06 \color{gray} $\pm$ 1.53 \color{black} & 2.02 \color{gray} $\pm$ 1.37 \color{black} & \textbf{\color{blue}1.55} \color{gray} $\pm$ 1.09 \color{black} & 4.12 \color{gray} $\pm$ 1.32\\
 
%  \color{black} & SAGE \color{black} & 18.04 \color{gray} $\pm$ 2.13 \color{black} & \textbf{\color{blue}2.22} \color{gray} $\pm$ 1.32 \color{black} & 16.78 \color{gray} $\pm$ 1.15 \color{black} & 2.35 \color{gray} $\pm$ 1.26 \color{black} & 2.34 \color{gray} $\pm$ 1.19 \color{black} & 3.32 \color{gray} $\pm$ 1.06\\
 
%  \color{black} & PEG \color{black} & 10.65 \color{gray} $\pm$ 0.72 \color{black} & 10.67 \color{gray} $\pm$ 1.03 \color{black} & 10.69 \color{gray} $\pm$ 1.12 \color{black} & 10.51 \color{gray} $\pm$ 0.98 \color{black} & 10.15 \color{gray} $\pm$ 1.09 \color{black} & \textbf{\color{blue}6.06} \color{gray} $\pm$ 0.89\\

%  % \color{black} & SEAL \color{black} &  \color{gray} $\pm$  \color{black} &  \color{gray} $\pm$  \color{black} &  \color{gray} $\pm$  \color{black} &  \color{gray} $\pm$  \color{black} &  \color{gray} $\pm$  \color{black} & \textbf{ \color{blue} \color{gray} $\pm$ }\\

%  \color{black} & GIN \color{black} & 18.29 \color{gray} $\pm$ 1.49 \color{black} & \textbf{\color{blue}2.74} \color{gray} $\pm$ 1.03 \color{black} & 17.89 \color{gray} $\pm$ 1.75 \color{black} & 2.81 \color{gray} $\pm$ 1.06 \color{black} & 2.93 \color{gray} $\pm$ 0.98 \color{black} & 6.20 \color{gray} $\pm$ 1.23\\

%  \color{black} & GCN \color{black} & 17.26 \color{gray} $\pm$ 2.15 \color{black} & 1.82 \color{gray} $\pm$ 1.26 \color{black} & 8.96 \color{gray} $\pm$ 1.18 \color{black} & 1.85 \color{gray} $\pm$ 1.15 \color{black} & \textbf{\color{blue}1.57} \color{gray} $\pm$ 0.98 \color{black} & 3.88 \color{gray} $\pm$ 1.92\\
 
\midrule 

 \parbox[t]{10mm}{\multirow{6}{*}{\rotatebox[origin=c]{0}{Chame}}}
 \color{black} & VGAE \color{black} & 7.52 \color{gray} $\pm$ 1.63 \color{black} & 2.83 \color{gray} $\pm$ 1.26 \color{black} & 6.39 \color{gray} $\pm$ 1.46 \color{black} & 2.84 \color{gray} $\pm$ 1.22 \color{black} & 2.77 \color{gray} $\pm$ 1.29 \color{black} & \textbf{ \color{blue}1.07} \color{gray} $\pm$ 0.34\\
 
 \color{black} & SAGE \color{black} & 5.98 \color{gray} $\pm$ 3.61 \color{black} & 3.46 \color{gray} $\pm$ 1.44 \color{black} & 12.0 \color{gray} $\pm$ 1.64 \color{black} & 3.59 \color{gray} $\pm$ 1.76 \color{black} & 3.23 \color{gray} $\pm$ 1.56 \color{black} & \textbf{\color{blue}2.46} \color{gray} $\pm$ 0.86\\

 \color{black} & PEG \color{black} & 4.44 \color{gray} $\pm$ 0.24 \color{black} & 2.84 \color{gray} $\pm$ 0.39 \color{black} & 2.28 \color{gray} $\pm$ 0.13 \color{black} & 2.82 \color{gray} $\pm$ 0.18 \color{black} & 2.44 \color{gray} $\pm$ 0.32 \color{black} & \textbf{\color{blue}1.66} \color{gray} $\pm$ 0.36\\

 % \color{black} & SEAL \color{black} &  \color{gray} $\pm$  \color{black} &  \color{gray} $\pm$  \color{black} &  \color{gray} $\pm$  \color{black} &  \color{gray} $\pm$  \color{black} &  \color{gray} $\pm$  \color{black} & \textbf{ \color{blue} \color{gray} $\pm$ }\\

 \color{black} & GIN \color{black} & 20.59 \color{gray} $\pm$ 1.96 \color{black} & 2.39 \color{gray} $\pm$ 1.23 \color{black} & 9.78 \color{gray} $\pm$ 1.08 \color{black} & 2.47 \color{gray} $\pm$ 1.17 \color{black} & 2.25 \color{gray} $\pm$ 1.31 \color{black} & \textbf{\color{blue}1.58} \color{gray} $\pm$ 0.97\\

 \color{black} & GCN \color{black} & 26.97 \color{gray} $\pm$ 1.94 \color{black} & 1.69 \color{gray} $\pm$ 0.96 \color{black} & 12.96 \color{gray} $\pm$ 1.63 \color{black} & \textbf{\color{blue}1.40} \color{gray} $\pm$ 0.97 \color{black} & 1.76 \color{gray} $\pm$ 0.95 \color{black} & 3.39 \color{gray} $\pm$ 0.92\\

 \color{black} & SEAL \color{black} & 3.21 \color{gray} $\pm$ 0.49 \color{black} & 2.67 \color{gray} $\pm$ 0.33 \color{black} & 2.64 \color{gray} $\pm$ 0.29 \color{black} & 3.31 \color{gray} $\pm$ 0.26 \color{black} & 2.98 \color{gray} $\pm$ 0.22 \color{black} & \textbf{ \color{blue}2.15} \color{gray} $\pm$ 0.32\\
 
\midrule

 \parbox[t]{7mm}{\multirow{6}{*}{\rotatebox[origin=c]{0}{Alpha}}}
 \color{black} & VGAE \color{black} & 20.36 \color{gray} $\pm$ 1.53 \color{black} & 9.42 \color{gray} $\pm$ 1.02 \color{black} & 10.89 \color{gray} $\pm$ 1.32 \color{black} & 8.71 \color{gray} $\pm$ 0.89 \color{black} & 8.65 \color{gray} $\pm$ 1.21 \color{black} & \textbf{\color{blue}8.42} \color{gray} $\pm$ 0.68\\
 
 \color{black} & SAGE \color{black} & 21.26 \color{gray} $\pm$ 1.37 \color{black} & 13.35 \color{gray} $\pm$ 1.02 \color{black} & 12.95 \color{gray} $\pm$ 1.31 \color{black} & 13.19 \color{gray} $\pm$ 1.13 \color{black} & 13.24 \color{gray} $\pm$ 1.40 \color{black} & \textbf{\color{blue}6.68} \color{gray} $\pm$ 0.91\\

 \color{black} & PEG \color{black} & 13.91 \color{gray} $\pm$ 1.13 \color{black} & 15.50 \color{gray} $\pm$ 1.09 \color{black} & 14.21 \color{gray} $\pm$ 1.16 \color{black} & 15.48 \color{gray} $\pm$ 2.02 \color{black} & 15.35 \color{gray} $\pm$ 1.03 \color{black} & \textbf{\color{blue}9.78} \color{gray} $\pm$ 0.89\\

 \color{black} & GIN \color{black} & 24.32 \color{gray} $\pm$ 2.63 \color{black} & 8.89 \color{gray} $\pm$ 1.12 \color{black} & 16.93 \color{gray} $\pm$ 1.63 \color{black} & 8.84 \color{gray} $\pm$ 1.36 \color{black} & 8.80 \color{gray} $\pm$ 1.17 \color{black} & \textbf{\color{blue}3.32} \color{gray} $\pm$ 0.89\\

 \color{black} & GCN \color{black} & 20.73 \color{gray} $\pm$ 1.75 \color{black} & 6.31 \color{gray} $\pm$ 1.97 \color{black} & 9.82 \color{gray} $\pm$ 1.19 \color{black} & 6.37 \color{gray} $\pm$ 1.58 \color{black} & 6.38 \color{gray} $\pm$ 1.67 \color{black} & \textbf{\color{blue}3.69} \color{gray} $\pm$ 1.98\\

   \color{black} & SEAL \color{black} & 2.60 \color{gray} $\pm$ 0.93 \color{black} & 3.68 \color{gray} $\pm$ 0.50 \color{black} & 3.25 \color{gray} $\pm$ 0.63 \color{black} & 3.41 \color{gray} $\pm$ 0.47 \color{black} & 3.39 \color{gray} $\pm$ 0.51 \color{black} & \textbf{\color{blue}2.04} \color{gray} $\pm$ 0.66\\
 
 \midrule

 \parbox[t]{7mm}{\multirow{6}{*}{\rotatebox[origin=c]{0}{OTC}}}
 \color{black} & VGAE \color{black} & 18.91 \color{gray} $\pm$ 1.62 \color{black} & 6.05 \color{gray} $\pm$ 1.19 \color{black} & 6.12 \color{gray} $\pm$ 0.98 \color{black} & 5.97 \color{gray} $\pm$ 0.69 \color{black} & \textbf{\color{blue}5.39} \color{gray} $\pm$ 0.87 \color{black} & 9.87 \color{gray} $\pm$ 0.97\\
 
 \color{black} & SAGE \color{black} & 24.04 \color{gray} $\pm$ 1.11 \color{black} & 13.00 \color{gray} $\pm$ 0.97 \color{black} & 14.58 \color{gray} $\pm$ 1.62 \color{black} & 12.86 \color{gray} $\pm$ 1.09 \color{black} & \textbf{\color{blue}12.68} \color{gray} $\pm$ 0.96 \color{black} & 15.09 \color{gray} $\pm$ 1.21\\

 \color{black} & PEG \color{black} & 12.89 \color{gray} $\pm$ 0.86 \color{black} & 11.94 \color{gray} $\pm$ 0.99 \color{black} & 9.62 \color{gray} $\pm$ 0.86 \color{black} & 12.03 \color{gray} $\pm$ 1.01 \color{black} & 12.09 \color{gray} $\pm$ 0.95 \color{black} & \textbf{\color{blue}6.35} \color{gray} $\pm$ 0.95\\
 
 \color{black} & GIN \color{black} & 20.01 \color{gray} $\pm$ 1.46 \color{black} & 2.55 \color{gray} $\pm$ 0.68 \color{black} & 12.96 \color{gray} $\pm$ 1.46 \color{black} & 2.08 \color{gray} $\pm$ 0.82 \color{black} & 2.02 \color{gray} $\pm$ 0.76 \color{black} & \textbf{\color{blue}1.23} \color{gray} $\pm$ 0.49\\

 \color{black} & GCN \color{black} & 20.55 \color{gray} $\pm$ 1.92 \color{black} & 5.46 \color{gray} $\pm$ 1.71 \color{black} & 10.34 \color{gray} $\pm$ 1.64 \color{black} & 5.34 \color{gray} $\pm$ 1.05 \color{black} & 5.42 \color{gray} $\pm$ 1.62 \color{black} & \textbf{\color{blue}4.88} \color{gray} $\pm$ 1.97\\

  \color{black} & SEAL \color{black} & 2.61 \color{gray} $\pm$ 0.89 \color{black} & 3.07 \color{gray} $\pm$ 0.62 \color{black} & 3.12 \color{gray} $\pm$ 0.74 \color{black} & 2.66 \color{gray} $\pm$ 0.70 \color{black} & 2.42 \color{gray} $\pm$ 0.62 \color{black} & \textbf{\color{blue} 2.19} \color{gray} $\pm$ 0.64\\

  \midrule

 \parbox[t]{7mm}{\multirow{2}{*}{\rotatebox[origin=c]{0}{DDI}}}
 \color{black} & VGAE \color{black} & 9.95 \color{gray} $\pm$ 1.24 \color{black} & 5.69 \color{gray} $\pm$ 0.63 \color{black} & 5.52 \color{gray} $\pm$ 0.75 \color{black} & 5.74 \color{gray} $\pm$ 0.90 \color{black} & 5.62 \color{gray} $\pm$ 0.81 \color{black} & \textbf{\color{blue}4.09} \color{gray} $\pm$ 0.99 \\

  \color{black} & PEG \color{black} & 9.04 \color{gray} $\pm$ 1.16 \color{black} & 6.39 \color{gray} $\pm$ 0.22 \color{black} & 6.59 \color{gray} $\pm$ 0.71 \color{black} & 6.54 \color{gray} $\pm$ 0.53 \color{black} & 6.51 \color{gray} $\pm$ 0.42 \color{black} & \textbf{\color{blue} 4.33} \color{gray} $\pm$ 0.48 \\

  \midrule

 \parbox[t]{7mm}{\multirow{2}{*}{\rotatebox[origin=c]{0}{Collab}}}
 \color{black} & VGAE \color{black} & 7.27 \color{gray} $\pm$ 0.73 \color{black} & 5.34 \color{gray} $\pm$ 0.43 \color{black} & 5.44 \color{gray} $\pm$ 0.52 \color{black} & 5.02 \color{gray} $\pm$ 0.49 \color{black} & 4.58 \color{gray} $\pm$ 0.62 \color{black} & \textbf{\color{blue}3.42} \color{gray} $\pm$ 0.58 \\

\color{black} & PEG \color{black} & 4.73 \color{gray} $\pm$ 0.81 \color{black} & 3.11 \color{gray} $\pm$ 0.52 \color{black} & 3.08 \color{gray} $\pm$ 0.56 \color{black} & 3.94 \color{gray} $\pm$ 0.30 \color{black} & 3.57 \color{gray} $\pm$ 0.46 \color{black} & \textbf{\color{blue}1.42} \color{gray} $\pm$ 0.35\\
\bottomrule
\end{tabular}
% }
\label{tab:ece_results}
\end{table*}

==> tables/gnn_performance.tex <==
\begin{table*}[!th]
\caption{\small GNN performances prior to calibration (mean and standard deviation for AUC, Hits@20 and ACC).}
\centering
\adjustbox{width=0.5\textwidth}{
\begin{tabular}{l l c c c c|}
\toprule
\textbf{Dataset} & \textbf{Model} & \textbf{AUC} & \textbf{Hits@20}& \textbf{ACC}\\ 
\cmidrule{1-5}

 \parbox[t]{7mm}{\multirow{6}{*}{\rotatebox[origin=c]{0}{cora}}}
 & VGAE & $89.79 \pm 0.50$ & $ 54.70\pm 4.40$ & $74.57 \pm 0.76$\\
 & SAGE & $87.93 \pm 1.68$ & $61.48 \pm 1.81$ & $75.23 \pm 1.74$\\
 & PEG & $88.01 \pm 1.76$ & $61.85 \pm 1.38$ & $71.06 \pm 1.25$ \\
 & GIN & $89.17 \pm 1.54$ & $52.18 \pm 1.16$ & $80.64 \pm 1.67$\\
 & GCN & $89.23 \pm 1.79$ & $62.80 \pm 1.72$ & $78.46 \pm 1.85$\\
 & SEAL & $91.24 \pm 0.89$ & $68.29 \pm 0.75$ & $79.68 \pm 0.83$\\
 
\midrule

 \parbox[t]{7mm}{\multirow{6}{*}{\rotatebox[origin=c]{0}{cite}}}
 & VGAE & $86.36 \pm 2.37$ & $50.95 \pm 5.21$ & $74.61 \pm 0.67$\\
 & SAGE & $84.89 \pm 1.47$ & $56.92 \pm 2.92$ & $72.19 \pm 1.89$\\
 & PEG & $90.57 \pm 1.62$ & $61.53 \pm 2.13$ & $70.65 \pm 1.49$\\
 & GIN & $82.47 \pm 1.76$ & $38.46 \pm 1.86$ & $78.90 \pm 1.81$\\
 & GCN & $82.24 \pm 1.91$ & $58.68 \pm 1.10$ & $76.37 \pm 1.67$\\
 & SEAL & $88.06 \pm 0.72$ & $67.28 \pm 0.91$ & $78.31 \pm 0.92$\\
 
\midrule

 \parbox[t]{7mm}{\multirow{6}{*}{\rotatebox[origin=c]{0}{pub}}}
 & VGAE & $95.37 \pm 0.37$ & $37.87 \pm 2.92$ & $75.49 \pm 0.64$\\
 & SAGE & $89.15 \pm 2.28$ & $41.85 \pm 1.99$ & $73.68 \pm 1.42$\\
 & PEG & $93.74 \pm 2.76$ & $44.35 \pm 1.13$ & $77.96 \pm 1.34$\\
 & GIN & $82.50 \pm 1.79$ & $26.96 \pm 1.24$ & $73.69 \pm 1.45$\\
 & GCN & $84.54 \pm 2.16$ & $37.65 \pm 2.12$ & $78.65 \pm 2.10$\\
 & SEAL & $96.81 \pm 0.26$ & $52.67 \pm 0.39$ & $82.97 \pm 0.34$\\
 
\midrule

 \parbox[t]{7mm}{\multirow{5}{*}{\rotatebox[origin=c]{0}{Twitch}}}
 & VGAE & $83.70 \pm 0.26$ & $19.47 \pm 0.24$ & $16.3 \pm 0.20$\\
 & SAGE & $88.03 \pm 0.68$ & $20.70 \pm 1.41$ & $69.34 \pm 0.84$\\
 & PEG & $91.68 \pm 0.72$ & $22.94 \pm 1.79$ & $84.69 \pm 0.91$\\
 & GIN & $87.64 \pm 1.21$ & $20.96 \pm 1.73$ & $65.85 \pm 1.12$\\
 % & SEAL & $ \pm $ & $ \pm $ & $ \pm $\\
 & GCN & $85.49 \pm 1.79$ & $24.89 \pm 2.03$ & $66.53 \pm 2.16$\\
 

\midrule

 \parbox[t]{7mm}{\multirow{6}{*}{\rotatebox[origin=c]{0}{chame}}}
 & VGAE & $97.22 \pm 1.17$ & $62.04 \pm 2.81$ & $58.70 \pm 1.63$\\
 & SAGE & $53.62 \pm 3.31$ & $23.8 \pm 0.88$ & $51.62 \pm 3.12$\\
 & PEG & $91.28 \pm 0.98$ & $46.67 \pm 0.82$ & $75.81 \pm 0.97$\\
  & GIN & $97.06 \pm 0.94$ & $71.45 \pm 1.08$ & $79.96 \pm 0.87$\\
 & GCN & $87.96 \pm 0.76$ & $13.26 \pm 1.96$ & $72.16 \pm 0.79$\\
 & SEAL & $98.12 \pm 0.54$ & $74.26 \pm 0.64$ & $82.13 \pm 0.44$\\
 
\midrule

 \parbox[t]{7mm}{\multirow{6}{*}{\rotatebox[origin=c]{0}{alpha}}}
 & VGAE & $81.91 \pm 2.21$ & $44.05 \pm 2.92$ & $64.37 \pm 2.26$\\
 & SAGE & $75.44 \pm 2.14$ & $37.46 \pm 1.23$ & $64.02 \pm 1.59$\\
  & PEG & $90.49 \pm 1.09$ & $47.87 \pm 1.19$ & $82.43 \pm 1.07$\\
 & GIN & $79.15 \pm 1.28$ & $41.50 \pm 1.27$ & $58.64 \pm 1.38$\\
 & GCN & $86.96 \pm 1.81$ & $45.32 \pm 1.97$ & $57.60 \pm 2.61$\\
 & SEAL & $93.91 \pm 0.41$ & $52.97 \pm 0.38$ & $87.28 \pm 0.54$\\

 \midrule

 \parbox[t]{7mm}{\multirow{6}{*}{\rotatebox[origin=c]{0}{OTC}}}
 & VGAE & $82.63\pm 2.76$ & $45.13 \pm 2.36$ & $64.02 \pm 2.53$\\
 & SAGE & $79.80 \pm 0.87$ & $44.48 \pm 0.67$ & $65.65 \pm 0.95$\\
 & PEG & $91.94 \pm 1.16$ & $59.56 \pm 1.05$ & $83.80 \pm 0.76$\\
 & GIN & $93.00 \pm 1.91$ & $46.39 \pm 1.98$ & $50.27 \pm 1.93$\\
 & GCN & $88.41 \pm 0.94$ & $44.62 \pm 1.87$ & $57.60 \pm 0.97$\\
 & SEAL & $95.94 \pm 0.61$ & $64.63 \pm 0.44$ & $84.34 \pm 0.62$\\

 \midrule

 \parbox[t]{7mm}{\multirow{2}{*}{\rotatebox[origin=c]{0}{DDI}}}
 & VGAE & $76.53 \pm 0.28$ & $37.12 \pm 0.14$ & $55.27 \pm 0.31$\\
 & PEG & $88.17 \pm 0.49$ & $39.07 \pm 0.20$ & $62.91 \pm 0.49$\\

  \midrule

 \parbox[t]{7mm}{\multirow{2}{*}{\rotatebox[origin=c]{0}{Collab}}}
 & VGAE & $72.26 \pm 0.46$ & $31.14 \pm 0.26$ & $46.81 \pm 0.44$\\
 & PEG & $85.57 \pm 0.42$ & $34.22 \pm 0.30$ & $48.09 \pm 0.39$\\
 
\bottomrule
\end{tabular}}
\label{tab:performanceGNN}
\vspace{-0.35cm}
\end{table*}

==> tables/his20_post.tex <==
\begin{table*}[thb]
% \onecolumn
\caption{Hits@20 post-calibration. \textbf{Hist} is the most harmful method for this metric while \texttt{IN-N-OUT} improves it in various scenarios. Here we highlight the worst values in \textcolor{red}{red}.}
\centering
% \vspace{4pt}
 % \resizebox{\textwidth}{!}{ 
\begin{tabular}{l l c c c c c c c c|}
\toprule 
\textbf{Datasets} \color{black} \color{black} & \textbf{Model} \color{black} \color{black} & \textbf{uncalibrated} \color{black} \color{black} & \textbf{Iso} \color{black} \color{black} & \textbf{Temp} \color{black} \color{black} & \textbf{BBQ} \color{black} \color{black} & \textbf{Hist} \color{black} \color{black} & \textbf{IN-N-OUT}\\ 
\midrule
 \parbox[t]{5mm}{\multirow{3}{*}{\rotatebox[origin=c]{0}{Cora}}} \color{black} & SAGE \color{black} &25.08 \color{gray} $\pm$ 1.81 \color{black} &22.46 \color{gray} $\pm$ 3.76 \color{black} &25.01 \color{gray} $\pm$ 1.81 \color{black} &21.12 \color{gray} $\pm$ 2.52 \color{black} &\textcolor{red}{15.42} \color{gray} $\pm$ 1.12 \color{black} &26.89 \color{gray} $\pm$ 1.19\\
 
 \color{black} & PEG \color{black} &67.32 \color{gray} $\pm$ 2.60 \color{black} &\textcolor{red}{51.63} \color{gray} $\pm$ 2.34 \color{black} &67.30 \color{gray} $\pm$ 2.60 \color{black} &54.01 \color{gray} $\pm$ 1.40 \color{black} &51.98 \color{gray} $\pm$ 1.89 \color{black} &68.37 \color{gray} $\pm$ 1.79\\
 
 % \color{black} & SEAL \color{black} &71.90 \color{gray} $\pm$ 0.71 \color{black} &70.23 \color{gray} $\pm$ 1.30 \color{black} &71.97 \color{gray} $\pm$ 0.71 \color{black} &71.55 \color{gray} $\pm$ 0.52 \color{black} &\bm{68.68 \color{gray} $\pm$ 0.78} \color{black} &74.68 \color{gray} $\pm$ 0.86\\
 
 \color{black} & GIN \color{black} &52.18 \color{gray} $\pm$ 1.16 \color{black} &37.00 \color{gray} $\pm$ 1.23 \color{black} &52.18 \color{gray} $\pm$ 1.16 \color{black} &30.17 \color{gray} $\pm$ 1.30 \color{black} &\textcolor{red}{24.28} \color{gray} $\pm$ 1.42 \color{black} &51.23 \color{gray} $\pm$ 1.63\\


 \midrule


 \parbox[t]{5mm}{\multirow{3}{*}{\rotatebox[origin=c]{0}{Citeseer}}}   \color{black} & SAGE \color{black} &38.09 \color{gray} $\pm$ 2.92 \color{black} &36.73 \color{gray} $\pm$ 3.50 \color{black} &38.06 \color{gray} $\pm$ 2.92 \color{black} &33.14 \color{gray} $\pm$ 4.36 \color{black} &\textcolor{red}{27.98} \color{gray} $\pm$ 10.1 \color{black} &40.15 \color{gray} $\pm$ 1.59\\
 
 \color{black} & PEG \color{black} &55.11 \color{gray} $\pm$ 1.59 \color{black} &53.68 \color{gray} $\pm$ 1.74 \color{black} &55.10 \color{gray} $\pm$ 1.59 \color{black} &55.16 \color{gray} $\pm$ 1.76 \color{black} &\textcolor{red}{53.44} \color{gray} $\pm$ 1.56 \color{black} &56.28 \color{gray} $\pm$ 1.61\\
 
 % \color{black} & SEAL \color{black} &72.45 \color{gray} $\pm$ 0.61 \color{black} &72.44 \color{gray} $\pm$ 1.63 \color{black} &72.43 \color{gray} $\pm$ 0.61 \color{black} &71.70 \color{gray} $\pm$ 0.87 \color{black} &\bm{70.91 \color{gray} $\pm$ 0.47} \color{black} &73.22 \color{gray} $\pm$ 0.69\\
 
 \color{black} & GIN \color{black} &38.46 \color{gray} $\pm$ 1.86 \color{black} &38.24 \color{gray} $\pm$ 1.45 \color{black} &38.46 \color{gray} $\pm$ 1.86 \color{black} &\textcolor{red}{32.08} \color{gray} $\pm$ 1.23 \color{black} &33.40 \color{gray} $\pm$ 1.62 \color{black} &38.45 \color{gray} $\pm$ 1.30\\ 

\midrule

 \parbox[t]{7mm}{\multirow{3}{*}{\rotatebox[origin=c]{0}{Alpha}}} \color{black} & SAGE \color{black} &44.97 \color{gray} $\pm$ 2.43 \color{black} &{39.87} \color{gray} $\pm$ 1.34 \color{black} &44.97 \color{gray} $\pm$ 2.43 \color{black} &43.48 \color{gray} $\pm$ 1.43 \color{black} & \textcolor{red}{37.39} \color{gray} $\pm$ 1.13 \color{black} &47.02 \color{gray} $\pm$ 1.09\\

 \color{black} & PEG \color{black} &49.29 \color{gray} $\pm$ 0.89 \color{black} &49.29 \color{gray} $\pm$ 0.91 \color{black} &49.29 \color{gray} $\pm$ 0.89 \color{black} &49.29 \color{gray} $\pm$ 0.96 \color{black} &\textcolor{red}{46.03} \color{gray} $\pm$ 1.01  \color{black} &49.29 \color{gray} $\pm$ 0.79\\
 
 \color{black} & GIN \color{black} &41.50 \color{gray} $\pm$ 1.27 \color{black} &39.73 \color{gray} $\pm$ 1.62 \color{black} &41.50 \color{gray} $\pm$ 1.27 \color{black} &42.91 \color{gray} $\pm$ 1.68 \color{black} &\textcolor{red}{38.17} \color{gray} $\pm$ 1.63 \color{black} &45.25 \color{gray} $\pm$ 1.40\\ 
\bottomrule
\end{tabular}
% }
\label{tab:hit20}
% \vspace{-0.35cm}
\end{table*}

==> tables/hits20_results.tex <==
\begin{table*}[!ht]
% \onecolumn
\caption{Hits@20 post-calibration. The lowest values are highlighted in red. \textbf{BBQ} and \textbf{Hits} are the most harmful methods for this metric. Importantly, \texttt{IN-N-OUT} improves both metrics in most cases ($>70$\%). Blue denotes cases in which \texttt{IN-N-OUT} improves Hits@20.}
\centering
% \resizebox{\textwidth}{!}{
\begin{tabular}{l l c c c c c c c c|}
\toprule
& \textbf{Model} & \textbf{uncalibrated} & \textbf{Iso} & \textbf{Temp} & \textbf{BBQ} & \textbf{Hist} & \textbf{IN-N-OUT}\\ 

\midrule

 \parbox[t]{5mm}{\multirow{6}{*}{\rotatebox[origin=c]{0}{cora}}}
 & VGAE & $54.70\pm 4.40$ & $50.89 \pm 4.27$ & $54.70 \pm 4.40$ & $49.34 \pm 4.67$ & \color{red}{$\bm{45.12 \pm 3.94}$} & \color{blue}{$55.62 \pm 3.15$}\\
 
 & SAGE & $61.48 \pm 1.81$ & $58.12 \pm 3.76$ & $61.48 \pm 1.81$ & $58.06 \pm 3.71$ & \color{red}{$\bm{49.93 \pm 2.76}$} & $61.17 \pm 2.72$\\
 
 & PEG & $61.85 \pm 1.38$ & $57.21 \pm 2.97$ & $61.85 \pm 1.38$ & $54.78 \pm 2.3$ & \color{red}{$\bm{52.98 \pm 1.89}$} & \color{blue}{$62.39 \pm 2.57$}\\
 
 & GIN & $52.18 \pm 1.16$ & $37.00 \pm 1.23$ & $52.18 \pm 1.16$ & $30.17 \pm 1.30$ & \color{red}{$\bm{24.28 \pm 1.42}$} & $51.23 \pm 1.63$\\

 & GCN & $62.80 \pm 1.72$ & $60.15 \pm 1.92$ & $62.80 \pm 1.72$ & $62.61 \pm 1.69$ & \color{red}{$\bm{57.68 \pm 1.39}$} & $62.42 \pm 1.21$\\

 & SEAL & $71.91 \pm 0.92$ & $70.20 \pm 0.98$ & $71.91 \pm 0.92$ & $71.53 \pm 0.85$ & \color{red}{$\bm{68.69 \pm 0.89}$} & $71.98 \pm 0.80$\\
 
\midrule

 \parbox[t]{5mm}{\multirow{6}{*}{\rotatebox[origin=c]{0}{cite}}}
 & VGAE & $50.95 \pm 5.21$ & $47.98 \pm 4.36$ & $50.95 \pm 5.21$ & $49.79 \pm 4.39$ & \color{red}{$\bm{43.18 \pm 4.87}$}  & \color{blue}{$52.15 \pm 3.97$}\\
 
 & SAGE & $56.92 \pm 2.92$ & $53.97 \pm 2.98$ & $56.92 \pm 2.92$ & $49.53 \pm 4.21$ & \color{red}{$\bm{35.75 \pm 4.13}$} & $56.89 \pm 2.13$\\
 
 & PEG & $61.53 \pm 2.13$ & $56.11 \pm 3.27$ & $61.53 \pm 2.13$ & $53.23 \pm 2.61$ & \color{red}{$\bm{51.14 \pm 2.48}$} & \color{blue}{$62.20 \pm 2.09$}\\
 
 & GIN & $38.46 \pm 1.86$ & $38.24 \pm 1.45$ & $38.46 \pm 1.86$ & \color{red}{$\bm{32.08 \pm 1.23}$} & $33.40 \pm 1.62$ & \color{blue}{$38.47 \pm 1.30$}\\

 & GCN & $58.68 \pm 1.10$ & $58.24 \pm 1.60$ & $58.68 \pm 1.10$ & $57.14 \pm 1.25$ & \color{red}{$\bm{47.47 \pm 1.62}$} & \color{blue}{$60.21 \pm 1.58$}\\

 & SEAL & $72.48 \pm 0.68$ & $72.48 \pm 0.71$ & $72.48 \pm 0.68$ & $71.72 \pm 0.93$ & \color{red}{$\bm{70.96 \pm 0.67}$} & $72.48 \pm 0.63$\\
 
\midrule

 \parbox[t]{5mm}{\multirow{6}{*}{\rotatebox[origin=c]{0}{pub}}}
 & VGAE & $37.87 \pm 2.92$ & $37.66 \pm 2.54$ & $37.87 \pm 2.92$ & $35.76 \pm 2.27$ & \color{red}{$\bm{0.00 \pm 0.00}$}  & \color{blue}{$38.12 \pm 2.25$}\\
 
 & SAGE & $41.85 \pm 1.99$ & $39.79 \pm 3.41$ & $41.85 \pm 1.99$ & $25.76 \pm 3.70$ & \color{red}{$\bm{23.86 \pm 4.10}$} & \color{blue}{$41.97 \pm 2.34$}\\
 
 & PEG & $44.35 \pm 1.13$ & $42.76 \pm 3.89$ & $44.35 \pm 1.13$ & $41.09 \pm 2.73$ & \color{red}{$\bm{0.00 \pm 0.00}$} & \color{blue}{$45.35 \pm 3.02$}\\
 
 & GIN & $26.96 \pm 1.24$ & $23.87 \pm 1.62$ & $26.96 \pm 1.24$ & $0.00 \pm 0.00$ & \color{red}{$\bm{0.00 \pm 0.00}$} & $26.92 \pm 1.63$\\

 & GCN & $37.65 \pm 2.12$ & $34.83 \pm 1.64$ & $37.65 \pm 2.12$ & $28.97 \pm 1.96$ & \color{red}{$\bm{0.00 \pm 0.00}$} & \color{blue}{$38.19 \pm 1.35$}\\

 & SEAL & $72.48 \pm 0.64$ & $72.48 \pm 0.68$ & $72.48 \pm 0.64$ & $70.96 \pm 0.63$ & \color{red}{$\bm{70.96 \pm 0.77}$} & $72.48 \pm 0.62$\\
 
\midrule

 \parbox[t]{5mm}{\multirow{5}{*}{\rotatebox[origin=c]{0}{Twitch}}}
 & VGAE & $19.47 \pm 0.24$ & $13.50 \pm 0.21$ & $19.42 \pm 0.24$ & $0.04 \pm 0.00$ & \color{red}{$\bm{0.04 \pm 0.00}$} & \color{blue}{$19.66 \pm 1.12$}\\
 
 & SAGE & $20.70 \pm 1.41$ & $9.49 \pm 2.18$ & $20.70 \pm 1.41$ & $0.00 \pm 0.00$ & \color{red}{$\bm{0.00 \pm 0.00}$} & \color{blue}{$20.28 \pm 1.14$}\\
 
 & PEG & $22.94 \pm 1.79$ & $21.72 \pm 1.34$ & $22.94 \pm 1.79$ & $0.00 \pm 0.00$ & \color{red}{$\bm{0.00 \pm 0.00}$} & $22.21 \pm 2.32$\\
 
 & GIN & $20.96 \pm 1.73$ & $18.66 \pm 1.53$ & $20.96 \pm 1.73$ & $20.54 \pm 1.42$ & \color{red}{$\bm{0.00 \pm 0.00}$} & \color{blue}{$21.09 \pm 1.50$}\\

 & GCN & $24.89 \pm 2.03$ & \color{red}{$\bm{23.45 \pm 1.43}$} & $24.89 \pm 2.03$ & $23.64 \pm 1.19$ & $24.16 \pm 1.26$ & $24.80 \pm 1.09$\\

\midrule

 \parbox[t]{7mm}{\multirow{6}{*}{\rotatebox[origin=c]{0}{chame}}}
 & VGAE & $62.04 \pm 2.81$ & $52.73 \pm 8.91$ & $62.02 \pm 2.81$ & $0.00 \pm 0.00$ & \color{red}{$\bm{0.00 \pm 0.00}$} & \color{blue}{$64.09 \pm 1.01$}\\
 
 & SAGE & $23.83 \pm 0.88$ & \color{red}{$\bm{19.14 \pm 2.40}$} & $23.80 \pm 0.88$ & $22.07 \pm 2.63$ & $22.26 \pm 3.05$ & $23.63 \pm 1.20$\\

 & PEG & $46.67 \pm 0.82$ & $45.96 \pm 1.58$ & $46.67 \pm 0.82$ & \color{red}{$\bm{42.73 \pm 2.03}$} & $42.87 \pm 1.90$  & \color{blue}{$47.23 \pm 2.34$}\\
 
 & GIN & $71.45 \pm 1.08$ & $68.33 \pm 1.34$ & $71.45 \pm 1.08$ & $71.24 \pm 1.97$ & \color{red}{$\bm{65.63 \pm 1.72}$} & \color{blue}{$72.56 \pm 1.25$}\\

 & GCN & $13.26 \pm 1.96$ & $11.03 \pm 1.57$ & $13.26 \pm 1.96$ & $0.00 \pm 0.00$ & \color{red}{$\bm{0.00 \pm 0.00}$} & $13.25 \pm 1.09$\\

 & SEAL & $74.26 \pm 0.64$ & $74.23 \pm 0.49$ & $74.26 \pm 0.64$ & $70.13 \pm 0.12$ & \color{red}{$\bm{69.78 \pm 0.19}$} & $74.26 \pm 0.53$\\
 
\midrule

 \parbox[t]{7mm}{\multirow{6}{*}{\rotatebox[origin=c]{0}{Alpha}}}
 & VGAE & $44.05 \pm 2.92$ & $44.01 \pm 3.41$ & $44.05 \pm 2.92$ & $40.91 \pm 2.72$ & \color{red}{$\bm{0.00 \pm 0.00}$} & \color{blue}{$44.96 \pm 2.19$}\\
 
 & SAGE & $37.46 \pm 1.23$ & $35.18 \pm 2.16$ & $37.46 \pm 1.23$ & $34.76 \pm 2.63$ & \color{red}{$\bm{21.34 \pm 2.34}$} & \color{blue}{$38.06 \pm 1.67$}\\

 & PEG & $47.87 \pm 1.19$ & $43.51 \pm 2.52$ & $47.87 \pm 1.19$ & $44.36 \pm 2.14$ & \color{red}{$\bm{34.72 \pm 2.63}$}  & \color{blue}{$47.89 \pm 1.86$}\\
 
 & GIN & $41.50 \pm 1.27$ & $39.73 \pm 1.62$ & $41.50 \pm 1.27$ & $42.91 \pm 1.68$ & \color{red}{$\bm{38.17 \pm 1.63}$} & \color{blue}{$45.25 \pm 1.40$}\\

 & GCN & $45.32 \pm 1.97$ & $44.33 \pm 1.92$ & $45.32 \pm 1.97$ & $44.61 \pm 1.92$ & \color{red}{$\bm{39.02 \pm 1.87}$} & \color{blue}{$45.49 \pm 1.93$}\\

 & SEAL & $52.97 \pm 0.66$ & $50.63 \pm 0.45$ & $52.97 \pm 0.66$ & \color{red}{$\bm{47.73 \pm 0.61}$} & $52.19 \pm 0.33$ & $52.97 \pm 0.5$\\
 
\midrule

 \parbox[t]{7mm}{\multirow{6}{*}{\rotatebox[origin=c]{0}{OTC}}}
 & VGAE & $45.13 \pm 2.36$ & $44.97 \pm 3.10$ & $45.13 \pm 2.36$ & $44.16 \pm 2.75$ & \color{red}{$\bm{40.03 \pm 1.97}$} & \color{blue}{$45.35 \pm 2.61$}\\
 
 & SAGE & $44.48 \pm 0.67$ & $42.09 \pm 2.19$ & $44.48 \pm 0.67$ & $35.91 \pm 1.89$ & \color{red}{$\bm{0.00 \pm 0.00}$} & \color{blue}{$44.52 \pm 1.09$}\\

 & PEG & $59.56 \pm 1.05$ & $54.95 \pm 0.96$ & $59.56 \pm 1.05$ & $53.09 \pm 1.06$ & \color{red}{$\bm{52.09 \pm 1.15}$}  & \color{blue}{$59.62 \pm 1.09$}\\
 
 & GIN & $46.39 \pm 1.98$ & $45.78 \pm 1.82$ & $46.39 \pm 1.98$ & $45.18 \pm 1.59$ & \color{red}{$\bm{41.46 \pm 1.57}$} & \color{blue}{$48.67 \pm 1.47$}\\

 & GCN & $44.62 \pm 1.87$ & $42.34 \pm 1.69$ & $44.62 \pm 1.87$ & $43.92 \pm 1.69$ & \color{red}{$\bm{39.92 \pm 1.67}$} & \color{blue}{$44.98 \pm 1.98$}\\

 & SEAL & $64.32 \pm 0.57$ & $63.94 \pm 0.41$ & $64.32 \pm 0.57$ & $64.32 \pm 0.48$ & \color{red}{$\bm{62.42 \pm 0.86}$} & $64.33 \pm 0.43$\\

\midrule

 \parbox[t]{7mm}{\multirow{2}{*}{\rotatebox[origin=c]{0}{DDI}}}
 & VGAE & $37.12 \pm 0.14$ & $35.16 \pm 0.20$ & $37.12 \pm 0.14$ & $36.19 \pm 0.22$ & \color{red}{$\bm{33.26 \pm 0.29}$} & $38.97 \pm 0.37$\\
 
 & PEG & $39.07 \pm 0.20$ & $38.55 \pm 0.47$ & $39.07 \pm 0.20$ & $37.19 \pm 0.51$ & \color{red}{$\bm{34.04 \pm 0.35}$} & $39.21 \pm 0.38$\\

\midrule

 \parbox[t]{7mm}{\multirow{2}{*}{\rotatebox[origin=c]{0}{Collab}}}
 & VGAE & $31.14 \pm 0.26$ & $31.14 \pm 0.29$ & $31.14 \pm 0.26$ & $31.09 \pm 0.32$ & \color{red}{$\bm{28.15 \pm 0.34}$} & $31.14 \pm 0.25$\\
 
 & PEG & $34.22 \pm 0.30$ & $32.11 \pm 0.65$ & $34.22 \pm 0.30$ & $32.59 \pm 0.51$ & \color{red}{$\bm{30.72 \pm 0.24}$} & $34.50 \pm 0.63$\\
\bottomrule
\end{tabular}
% }
\label{tab:hit20app}
% \vspace{-0.35cm}
\end{table*}

==> tables/teste_hipotese.tex <==
\begin{table}[hbtp!]
\caption{Wilcoxon’s sign rank tests \(\alpha = 5\%\).} 
\centering
\resizebox{\linewidth}{!}{


\adjustbox{width=\linewidth}{
\begin{tabular}{lccccccc}
\toprule

\textbf{} & \textbf{cora} & \textbf{cite}  & \textbf{pub} & \textbf{twitch} & \textbf{chame} & \textbf{alpha} & \textbf{otc}\\ 
\toprule
VGAE & {\color{blue} \checkmark} & \xmark & {\color{blue} \checkmark} & {\color{blue} \checkmark} & {\color{blue} \checkmark} & \xmark &  \\
SAGE & {\color{blue} \checkmark} & {\color{blue} \checkmark} & {\color{blue} \checkmark} & \xmark & \xmark & {\color{blue} \checkmark} &  \\
PEG & {\color{blue} \checkmark} & {\color{blue} \checkmark} & {\color{blue} \checkmark} & {\color{blue} \checkmark} & {\color{blue} \checkmark} & {\color{blue} \checkmark} & {\color{blue} \checkmark} \\
GIN & {\color{blue} \checkmark} & {\color{blue} \checkmark} & {\color{blue} \checkmark} &  & {\color{blue} \checkmark} & {\color{blue} \checkmark} & {\color{blue} \checkmark} \\
GCN & {\color{blue} \checkmark} & {\color{blue} \checkmark} &  &  &  & \xmark & \xmark \\

\bottomrule
\end{tabular}

}

}
\label{tab:hipotese}
% \vspace{-0.35cm}
\end{table}
